Cluster structures in Schubert varieties in the Grassmannian

In this article we explain how the coordinate ring of each (open) Schubert variety in the Grassmannian can be identified with a cluster algebra, whose combinatorial structure is encoded using (target labelings of) Postnikov's plabic graphs. This result generalizes a theorem of Scott (Scott 2006) for the Grassmannian, and proves a folklore conjecture for Schubert varieties that has been believed by experts since (Scott 2006), though the statement was not formally written down until M\"uller-Speyer explicitly conjectured it (M\"uller-Speyer 2016). To prove this conjecture we use a result of Leclerc (Leclerc 2016), who used the module category of the preprojective algebra to prove that coordinate rings of many Richardson varieties in the complete flag variety can be identified with cluster algebras. Our proof also uses a construction of Karpman (Karpman 2016) to build plabic graphs associated to reduced expressions. We additionally generalize our result to the setting of skew Schubert varieties; the latter result uses generalized plabic graphs, i.e. plabic graphs whose boundary vertices need not be labeled in cyclic order.

==> FactorizationLemma.tex <==
%This is the lemma about the correspondence between permutations with length-additive factorizations w=xv and pairs of lattice paths in a k x (n-k) rectangle


Fix $n \in \Z_+$ and $k\leq n$. As usual, $s_i$ denotes the simple transposition $(i ~ i+1)$, $W_K$ denotes the parabolic subgroup generated by $\set{s_1, \dots, s_{n-1}} \setminus \set{s_k}$, $w_K$ the longest element of this parabolic subgroup, and $W^K$  and $^K W$ ($W^K_{max}$  and $^K _{max} W$) denote the set of minimum (maximum) length left and right coset representatives of $W_K$, respectively. We associate to each $k$-subset $I$ of $[n]$ a lattice path from the southwest corner of a $k \times (n-k)$ rectangle to the northeast corner whose vertical steps are $I$. Let $I=\set{i_1 < \cdots < i_k}$ and $J=\set{j_1 < \cdots <j_k}$ be subsets of $[n]$. $I \leq J$ if $i_r \leq j_r$ for all $r$; in this case, $I$ lies ``above" $J$ when drawn in the rectangle. 

\begin{lem} Let $\A \subseteq S_n$ consist of permutations $w$ that have a length additive factorization $w=xv$, where $v \in {^K _{max}W}$. Then there is a surjection
\[ \beta: \{(I, J)| I, J \in \binom{[n]}{k} \text{ and }I \leq J\} \to \A.
\]
\end{lem}
 \begin{proof} First, note that if $w \in \A$ with factorization $xv$, then $x \in W^K$. We will first describe how to obtain $x_I$ and $v_J$ from $I$ and $J$ (thinking of the subsets as lattice paths), and then will show by induction on the number of boxes below $J$ that $\beta: (I, J) \mapsto x_I v_J$  is well-defined.
 
 To obtain $x_I$, we number the steps of $I$ with $1, 2, \dots, n$, starting at the southwest corner and going to the northeast corner. $x_I(a)$ is the label of the $a^{th}$ vertical step if $a\leq k$ and is the label of the $(a-k)^{th}$ horizontal step if $a > k$. To obtain $v_J$, we number the vertical steps of $J$ with $1, \dots, k$, going from southwest corner to northeast corner, and number the horizontal steps with $k+1, \dots, n$. If we read this path from northeast corner to southwest corner, it gives $v_J$ in one-line notation. Note that $x_I \in W^K$ and $v_J \in {^K _{max} W}$. 
 
 When $J=\{n-k+1, \dots, n\}$, $v_J=w_K$. Further, $x_I w_K$ is length-additive for all $I$, as $x_I \in W^K$.
 
 Now, fix $I$ and suppose $I \leq J$. We will show that if a lattice path $M$ is obtained from $J$ by adding a box $m$ above $J$, then $l(x_I v_M) > l(x_I v_J)$ if and only if $m$ is not above $I$. 

Suppose $v_J(a)=b$ and $v_J(a+1)=c$. Then $s_a$ is a right ascent of $x_I v_J$ if and only if $b \leq k$, $c>k$, and the label of the $b^{th}$ vertical step of $I$ is smaller than the label of the $(c-k)^{th}$ horizontal step of $I$. The first two conditions are equivalent to the $a^{th}$ step of $J$ being vertical and the $(a+1)^{th}$ horizontal; the third means that the $b^{th}$ vertical step of $I$ comes before the $(c-k)^{th}$ horizontal step of $I$.


Note that since $M$ is a lattice path, the east and south edges of $m$ are in $J$, say the $j^{th}$ and $(j+1)^{th}$ steps. Then $v_M=v_J s_j$, so it suffices to show that $s_j$ is a right ascent of $x_I v_J$ if and only if $m$ is not above $I$. Let $v_J(j)=b$ and $v_J(j+1)=c$. The condition that the $j^{th}$ step and the $(j+1)^{th}$ step of $J$ are vertical and horizontal, respectively, is always satisfied. If the $b^{th}$ vertical step of $I$ comes before the $(c-k)^{th}$ horizontal step of $I$, then this means precisely that $m$ is below $I$, since the $j^{th}$ step of $J$ is $b$ vertical steps from the south edge of the rectangle and the $(j+1)^{th}$ step of $J$ is $(c-k)$ horizontal steps from the west edge of the rectangle. Conversely, if the $b^{th}$ vertical step of $I$ comes after the $(c-k)^{th}$ horizontal step of $I$, then $m$ is above $I$.

 
This shows that $\beta$ is well-defined: if $I \leq M$, and $J$ is a lattice path obtained from $M$ by removing a box $m$ below $M$, then $I \leq J$ so $x_I v_J$ is length-additive by induction. Since $m$ is not above $I$ by assumption, $l(x_I v_M) > l(x_I v_J)$ and thus $x_I v_M$ is length-additive.

 Surjectivity follows from $\beta$ being well-defined. If $w \in \A$ with length-additive factorization $xv$, we associate to $x$ the lattice path $I$ with vertical steps at $x([k])$, going from southwest corner to northeast. We associate to $v$ the lattice path $J$ with vertical steps at $v^{-1}([k])$, going from northeast corner to southwest. It's clear that $x_I=x$ and $v_J=v$. 
 
To show that $I \leq J$, we build up $J$ box by box. Note that if the $a^{th}$ step of $J'$ is vertical and the $(a+1)^{th}$ is horizontal, then $s_a$ is a right ascent of $v_{J'}$ and adding a box next to the $a^{th}$ and $(a+1)^{th}$ steps produces the lattice path associated to $v_{J'}s_a$. So the length of $v$ is $l(w_K)$ plus the number of boxes below $J$. This means that when building up $J$, if in some step we have $J'$, the box we add above $J'$ must correspond to a right ascent of $x v_{J'}$; if it is instead a descent, then $l(xv)<l(x) + l(v)$. By the argument above, this is equivalent to all of the boxes below $J$ being below $I$ as well.
 
 \end{proof}


==> Lemma.tex <==
%\begin{definition} Let $w \in S_n$. If $w=xv$ and $\ell(w)=\ell(x)+\ell(v)$, we say that $xv$ is a \emph{length-additive factorization} of $w$.
%\end{definition}


Let $J, L$ be lattice paths from $(0, 0)$ to $(n-k, k)$ taking steps north and east and suppose $\vertne{J}=\set{j_1 < \cdots < j_k}$ and $\vertne{L}=\set{l_1 < \cdots <l_k}$. We say $J \leq L$ if $j_r \leq l_r$ for all $r$; that is, $J$ ``lies above'' $L$ when drawn in the plane. 

\begin{lemma} \label{prop:lengthsadd} Let $\A=\{(v, w)\ \vert \ v \in W^K_{\max}, w\in W \text{ with length-additive factorization } w=xv\}$. The following map is a bijection:
\begin{align*} \A &\to \{(J, L)\ \vert \  J \leq L \text{ lattice paths from } (0, 0) \text{ to }(n-k, k)\}\\
(v, xv) & \mapsto (\pathne{x([k])}, \pathsw{v^{-1}([k])}).
\end{align*}
\end{lemma}
 \begin{proof} 
 For convenience, we first give a well-defined map $\beta:(J, L) \mapsto (v_L, x_J v_L)$ in the opposite direction, and then show that the map in the proposition is well-defined and the inverse of $\beta$.
 
Note that if $w$ has length-additive factorization $xv$ with $v\in W^K_{\max}$, then necessarily $x \in {^K W}$. In what follows, it will matter which direction one labels and reads the labels of a lattice path $L$. The notation $L^\nearrow$ (resp. $L^\swarrow$) indicates one should label or read the path going northeast (resp. southwest). 

Fix lattice paths $J \leq L$. To obtain $x_J$ in list notation, label $J^\nearrow$ with $1, \dots, n$. Read the labels of the vertical steps of $J^\nearrow$ and then read the labels of the horizontal steps. To obtain $v_L$ in list notation, label the vertical steps of $L^\nearrow$ with $1, \dots, k$ and label the horizontal steps with $k+1, \dots, n$. Then read the labels of $L^\swarrow$. To show that $x_J v_L$ is length-additive, we proceed by induction on $\ell(v_L)$

Note that $x_J \in {^K W}$ and $v_L \in W^K_{\max}$.
When $\vertne{L}=\{n-k+1, \dots, n\}$, 
%\Comment{Kh: instead of $L$ write $V^\nearrow(L)$?}
$v_L=w_K$ and $x_J w_K$ is length-additive for all $J$. 
%\Comment{Kh: this should be $^K W$?}
 
Now, fix $J$ and suppose $J \leq L$. Let $M$ be a lattice path obtained from $L$ by adding a box $m$ above $L$. Say the east and south edge of $m$ are the $l^{th}$ and $(l+1)^{th}$ steps in $L^\swarrow$, respectively; then $v_M=v_L s_l$.

Suppose $v_L(l)=p$ and $v_L(l+1)=q$. It follows from the definitions that $s_l$ is a right ascent of $x_J v_L$ (that is, $\ell(x_J v_Ls_l)=\ell(x_J v_L)+1$)  
%\Comment{Kh: it would be good to say what is meant by right ascent, I did not know this term} 
if and only if 
%$b \leq k$, $c>k$, and the label of the $b^{th}$ vertical step of $J^\nearrow$ is smaller than the label of the $(c-k)^{th}$ horizontal step of $J^\nearrow$. The first two conditions are equivalent to the $a^{th}$ step of $L^\swarrow$ being vertical and the $(a+1)^{th}$ horizontal, which is always satisfied; the third means that 
the $p^{th}$ vertical step of $J^\nearrow$ comes before the $(q-k)^{th}$ horizontal step of $J^\nearrow$. Note that the $l^{th}$ step of $L^\swarrow$ is $p$ vertical steps from the south edge of the rectangle and the $(l+1)^{th}$ step of $L^\swarrow$ is $(q-k)$ horizontal steps from the west edge of the rectangle. This means that $m$ is below $J$ if and only if the $p^{th}$ vertical step of $J^\nearrow$ comes before the $(q-k)^{th}$ horizontal step of $J^\nearrow$. So $\ell(x_J v_M) > \ell(x_J v_L)$ if and only if $m$ is not above $J$. 

 
From this we can conclude that $\beta$ is well-defined. Indeed, suppose $J \leq M$ and $L$ is the lattice path obtained from $M$ by removing a box $m$ below $M$. Then $J \leq L$ so $x_J v_L$ is length-additive by induction. Since $m$ is not above $J$ by assumption, $\ell(x_J v_M) >\ell(x_J v_L)$ and thus $x_J v_M$ is length-additive.


We define the inverse of $\beta$ as follows. If $(v, w)\in \A$ and $w=xv$ is length-additive, we associate to $x$ the lattice path $J:=\pathne{x([k])}$ and associate to $v$ the lattice path $L:=\pathsw{v^{-1}([k])}$. It is apparent from the definitions that $x_J=x$ and $v_L=v$.
 
To show that $J \leq L$, we build up $L$ box by box. 
%Note that if the $a^{th}$ step of a lattice path $\tilde{L}^\swarrow$ is vertical and the $(a+1)^{th}$ is horizontal, then $s_a$ is a right ascent of $v_{\tilde{L}}$. Adding a box next to the $a^{th}$ and $(a+1)^{th}$ steps produces the lattice path associated to $v_{\tilde{L}}s_a$.
Note that the length of $v=v_L$ is $\ell(w_K)$ plus the number of boxes below $L$. This means that when building up $L$, if in some step we have $\tilde{L}$, the box $m$ we add above $\tilde{L}$ must correspond to a right ascent of $x v_{\tilde{L}}$; otherwise we would have $\ell(xv) < \ell(x)+\ell(v)$. By the argument above, this is equivalent to the box $m$ being below $J$. Thus, all boxes below $L$ are also below $J$ and $J \leq L$.
 \end{proof}


 
 
 
 
 
 


==> oldconclusion.tex <==


In this section we give applications of \cref{thm:main} and \cref{thm:main2},
and also give a conjectural generalization of \cref{thm:main2} to arbitrary positroids.



\subsection{The coordinate rings of Schubert and skew-Schubert varieties}\label{sec:skew}

Combining \cref{thm:main} and \cref{thm:main2} with
\cite[Theorem 3.3]{MullerSpeyer0} and \cite{Muller}, 
we find that the coordinate rings of Schubert and skew Schubert varieties (viewed as cluster algebras) are \emph{locally acyclic},
which implies that they are finitely generated, normal, locally a complete
intersection, and equal to their own upper cluster algebras.

Combining our result with \cite[Theorem 1.2]{FordSer}, 
we find that the quivers giving
rise to the cluster structures for Schubert and skew Schubert varieties admit
\emph{green-to-red sequences}, which by \cite{GHKK} implies that the cluster algebras have
\emph{Enough Global Monomials} and hence 
each coordinate ring has a canonical basis of
\emph{theta functions}, parameterized by the lattice of $g$-vectors.



\subsection{Schubert varieties whose cluster structure has finite type}

Recall that there is a simple way to obtain a cluster seed from the 
Young diagram indexing a Schubert variety, see \cref{PPQ}.


\begin{figure}[h]
\centering
\includegraphics[height=2in]{Partition-Plabic-Quiver.pdf}
\caption{The plabic graph and quiver associated to Young diagram.}
\label{PPQ}
\end{figure}

In \cite{Scott}, Scott classified the Grassmannians whose coordinate rings
have a cluster algebra of finite type.  He showed that in general the
cluster algebras have infinite type, except in the following cases:
the coordinate ring of $Gr_{2,n}$ has a cluster algebra of type $A_{n-3}$,
while the coordinate rings of $Gr_{3,6}$, $Gr_{3,7},$ and $Gr_{3,8}$ have
cluster algebras of types $D_4$, $E_6$, and $E_8$, respectively.

It is straightforward to classify for which positroid varieties $\pi_k(\mathcal{R}_{v, w})$ (where $\ell(w)=\ell(v)+\ell(wv^-1)$) the cluster structure described here is finite type. It depends only on $wv^{-1}$. We will need the following two facts. 

\begin{proposition}[\Comment{cite Keller}] \label{prop:sametree} Let $Q$ and $Q'$ be two acyclic quivers. If $Q$ can be obtained from $Q'$ by a sequence of mutations, then $Q$ and $Q'$ are orientations of isomorphic trees.
\end{proposition}

\begin{lemma}\label{lem:infinitesubquiver} Let $Q$ be a quiver and $Q'$ a subquiver of $Q$. If $Q'$ is not a quiver of finite type \Comment{possibly add: (that is, one cannot obtain an orientation of a type ADE Dynkin diagram from $Q'$ by a sequence of mutations)}, then $Q$ is not a quiver of finite type.
\end{lemma}

\begin{proposition} Let $v \leq w$, where $v \in W^K_{\max}$ and $w=xv$ is length-additive. Let $\lambda=\partne{x([k])}$ and let $\lambda'$ be the diagram obtained from $\lambda$ by removing the boxes that correspond to frozen vertices in the quiver $Q_{v, w}$ (see \cref{def:labeledquiver}). Let $\A := \A(Q_{v, w})$, where the labeled quiver $Q_{v, w}$ is considered as a seed.

\begin{enumerate}
\item $\A$ is type $A$ if and only if $\lambda'$ does not contain a $2 \times 2$ rectangle.
\item $\A$ is type $D$ if and only if $\lambda'=(i, 2)$ or its transpose for $i \geq 2$.
\item $\A$ is of type $E_6$, $E_7$, or $E_8$ if and only if $\lambda'$ is one of the shapes shown in \cref{fig:exceptionaltypes}.
\end{enumerate}

\end{proposition}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{exceptionalTypes2}
\caption{\label{fig:exceptionaltypes}Up to transposition, the smallest partitions giving rise to quivers of types $E_6, E_7, E_8$, whose mutable vertices are shown on the right. The boxes corresponding to mutable vertices are colored green. Adding any number of boxes to the first row or column of these partitions only adds frozen vertices to the quiver, and so also gives rise to a quiver of type $E_6, E_7, E_8$.}
\end{figure}

\begin{proof}
\begin{enumerate}
\item The backwards direction follows from the fact that if $\lambda'$ does not contain a $2 \times 2$ rectangle, then $Q_{v, w}$ is an orientation of a path. For the other direction, recall that the mutable part of all type A quivers can be obtained from a triangulation of a polygon \Comment{insert reference?}. It is not hard to see that there is no arrangement of 4 arcs in a triangulation that gives the quiver we draw from a $2 \times 2$ rectangle according to \cref{def:labeledquiver}, so if $\lambda'$ contains a $2 \times 2$ rectangle as a subdiagram, $\A$ is not type $A$.
\item The backwards direction follows from inspection of the associated quivers; if one mutates at the vertex in the northwest box, one obtains an orientation of a type $D$ Dynkin diagram. If $|\lambda'|\leq 8$, then necessity follows from direct computation and \cref{prop:sametree}. Four partitions of $8$ are not finite type (see \cref{fig:mininfinite}), so by \cref{lem:infinitesubquiver} any partition containing one of these four will not be finite type. The partitions of $9$ that are not of type $A$, are not $(7, 2)$ or its transpose, and do not contain a partition of 8 that is infinite type are shown in \cref{fig:mininfinite}; they are all infinite type. Thus, the only partitions of $9$ that are finite type and not type $A$ are $(7, 2)$ and its transpose. From this, we can conclude that $\A$ is type $D$ only if $\lambda'=(i, 2)$ or its tranpose. Indeed, $\A$ is infinte type if $\lambda'$ is not type $A$ and contains any partition of $9$ that is not $(7, 2)$ or its transpose, or, equivalently, if $\lambda\neq(i, 2)$ or its transpose. 
\item By direct computation, using the fact that if two acyclic quivers are mutation-equivalent then they are orientations of isomorphic trees.
\end{enumerate}
\end{proof}


\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{minInfinite}
\caption{\label{fig:mininfinite} These partitions (and their transposes) are the smallest partitions giving rise to quivers of infinite type, whose mutable vertices are shown on the right. The boxes corresponding to mutable vertices are shown in green. Adding any number of boxes to the first row or column of these partitions only adds frozen vertices to the quiver, and so also gives rise to a quiver of infinite type.}
\end{figure}


\begin{cor} Let $\lambda$ be a partition fitting inside a $k \times (n-k)$ rectangle. Then the cluster structure on $X_\lambda \subseteq Gr_{k, n}$ given in \cref{thm:main} is finite type if and only if

\begin{itemize}
\item $\lambda$ contains a $2 \times 2$ rectangle but not a $3 \times 3$ rectangle (type $A$);
\item $\lambda$ contains a $3 \times 3$ rectangle but not a $4 \times 3$ rectangle (type $D$, see \cref{FinType});
\item $\lambda$ is one of the shapes shown in \cref{fig:exceptionaltypes} (types $E_6$, $E_7$, $E_8$).
\end{itemize}
\Comment{check to make sure these descriptions match what we actually mean.}
\end{cor}

%In particular, we can find realizations of type $D_n$ as well as $E_7$ 
%cluster algebras in the coordinate rings of Schubert varieties, see 
%\cref{FinType}.

\begin{figure}[h]
\centering
\includegraphics[height=.9in]{FiniteTypeSchubert}
\caption{A series of Schubert varieties which yield the type 
	$D_n$ cluster algebras.}
\label{FinType}
\end{figure}



\subsection{Applications to the preprojective algebra}

As an application of Theorem~\ref{thm-module-structure}, we obtain an explicit way to compute the summands of a cluster-tilting module $U_{v,w}$, whereas Lecler'c definition is constructive.  This provides a novel connection between Pl{\"u}cker coordinates and the structure of the summands of $U_{v,{\bf w}}$.  It is an interesting problem to determine whether this correspondence extends beyond the case of Schubert and skew-Schubert varieties.   Such combinatorial interpretation of the modules would be useful in computing morphisms between the summands of $U_{v,{\bf w}}$ for arbitrary $(v,{\bf w})$.  Moreover, given two modules $U, U' \in \mathcal{C}_{v,w}$ that correspond to Pl{\"ucker} coordinates $\Delta_{P}, \Delta_{P'}$ on the positroid variety $\overline{\pi_k(\mathcal{R}_{v,w})}$, it is natural to ask whether we can detect an extension between $U$ and $U'$ in terms of the corresponding lattice paths $\pathsw{P}, \pathsw{P'}$.  In particular, this would tell us whether two cluster variables $\Delta_{P}, \Delta_{P'}$ are compatible in the cluster algebra $\mathbb{C}[\mathcal{R}_{v,w}]$.  
This can provide new insights into the representation theory of preprojective algebras, that are an important ingredient in studying cluster algebras related to semisimple algebraic groups.

Moreover, when $w=xv$ is a length additive factorization and $v\in W^K_{max}$, we explicitly write down 
some of the seeds for the pair $(v,w)$, and identify them with the seeds coming from reduced 
plabic graphs.  
Thus we find that these cluster algebras have all the nice properties
 mentioned in \cref{sec:skew} (they are locally acyclic, equal to their upper cluster algebra,
 admit green-to-red sequences, have a canonical
 basis of theta functions, etc).


\subsection{The conjecture for positroid varieties}

We believe that \cref{thm:main2} extends to arbitrary positroid
varieties as follows.

\begin{conjecture}\label{conj:pos}
Choose $w\in W$ and $v\in W^K_{max}$ where
$v \leq w$.
  Let $G$ be a reduced plabic graph
(with boundary vertices labeled clockwise from $1$ to $n$) with
        trip permutation $vw^{-1}$, and such that boundary lollipops
are white if and only if they are in $[k]$. Then the coordinate
ring of the (affine cone over) the positroid
	variety $P_x \equiv \overline{\mathcal{R}_{v,w}}$ is a cluster algebra, and $G$ gives rise to a seed as follows:
we  relabel boundary vertices of $G$ by $v^{-1}$ and apply
the target labeling.  This gives a labeling by Pl\"ucker coordinates of
 the dual quiver of $G$.
\end{conjecture}

We note that outside of the Schubert setting, \cref{conj:pos} differs from \cref{conj:vague}.
More specifically, the plabic graphs from \cref{conj:vague} have boundary vertices labeled in order from 
$1$ to $n$, while the graphs in \cref{conj:pos} have boundary vertices labeled in order 
by the entries of $v^{-1}$.  

